Integrating On-demand Ride-sharing with Mass Transit at-Scale

We are in the midst of a technology-driven transformation of the urban mobility landscape. However, unfortunately these new innovations are still dominated by car-centric personal mobility, which leads to concerns such as environmental sustainability, congestion, and equity. On the other hand, mass transit provides a means to move large amounts of travelers very efficiently, but is not very versatile and depends on an adequate concentration of demand. In this context, our overarching goal is to explore opportunities for new technologies such as ride-sharing to integrate with mass transit and provide a better service. More specifically, we envision a hybrid system that uses on-demand shuttles in conjunction with mass transit to move passengers efficiently, and provide an algorithmic framework for operational optimization. Our approach extends a state-of-the-art trip-vehicle assignment model to the multi-modal setting, where we develop a new integer-linear programming formulation to solve the problem efficiently. A comprehensive study covering five major cities in the United States based on real-world data is carried out to verify the advantages of such a system and the effectiveness of our algorithms. We show that our hybrid system provides significant improvements in comparison to a purely on-demand model by exploiting the efficiencies of the mass transit system.

==> graphs/DIS.tex <==
\begin{figure*}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    title={Capacity=1},
    xlabel={No of Vehicles},
    ylabel={Precentage (\%)},
    % xmin=500, xmax=2000,
    ymin=0, ymax=60,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={0,20,40,60,80,100},
    legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    label style={font=\small},
    tick label style={font=\small},
    % title style={at={(0,1)}}
]

\addplot[
    color=black,
    mark=square
    ]
    coordinates {
    (1,41.32)(2,50.16)(3,49.91)
    };

\addplot[
    color=black,
    mark=*,
    style=densely dotted,
    ]
    coordinates {
    (1,8.57)(2,8.77)(3,13.26)
    };

\addplot[
    color=black,
    mark=x,
    style=dashed,
    ]
    coordinates {
    (1,50.11)(2,41.07)(3,36.83)
    };


\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    title={Capacity=2},
    xlabel={No of Vehicles},
    % ylabel={Precentage (\%)},
    % xmin=500, xmax=2000,
    ymin=0, ymax=60,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={0,20,40,60,80,100},
    legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    label style={font=\small},
    tick label style={font=\small},
    % title style={at={(0,1)}}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,46.6)(2,51.87)(3,50.79)
    };
% \addlegendentry{Multi Cap 2}

\addplot[
    color=black,
    mark=*,
    style=densely dotted,
    ]
    coordinates {
    (1,9.66)(2,12.25)(3,13.18)
    };
% \addlegendentry{Multi Cap 4}

\addplot[
    color=black,
    mark=x,
    style=dashed,
    ]
    coordinates {
    (1,43.73)(2, 35.88)(3,36.02)
    };
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    title={Capacity=4},
    xlabel={No of Vehicles},
    % ylabel={Precentage (\%)},
    % xmin=500, xmax=2000,
    ymin=0, ymax=60,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={0,20,40,60,80,100},
    % legend pos=outer north,
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    label style={font=\small},
    tick label style={font=\small},
    custom legend,
    legend style={at={(1,1.2)},anchor=south east,
        column sep=0.5em},
    % title style={at={(0,1)}}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,49.21)(2,52.78)(3,51.72)
    };
    
\addplot[
    color=black,
    mark=*,
    style=densely dotted,
    ]
    coordinates {
    (1,9.64)(2,12.25)(3,13.1)
    };
    
\addplot[
    color=black,
    mark=x,
    style=dashed,
    ]
    coordinates {
    (1,41.15)(2,34.97)(3,35.19)
    };
% \addlegendentry{MOD Cap 4}
\legend{Ride-Sharing-Only, Transit-Only,Multi-Modal}
\end{axis}
\end{tikzpicture}

\caption{Describes the distribution of trip composition for all the served trips in the Multi-modal settings for varying vehicle capacities (1,2 and 4) and fleet sizes (500,1000,2000). MoD-only and bus-only trips are the trips that are solely served by MoD vehicles or buses respectively. Bus-MoD trips are served by a combination of buses and MoD vehicles. Plot (A),(B), and (C) represent capacities 1,2 and 4 respectively.}
\label{fig:composition}
\end{figure*}

==> graphs/EXE.tex <==
\begin{figure*}[ht]

% \centering
\rotatebox{90}{\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,(A) VMT}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    title={Capacity=1},
    xlabel={No of Vehicles},
    ylabel={KMs},
    % xmin=500, xmax=2000,
    ymin=1,ymax=6.5,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={1,1.5,2,2.5,3,3.5,4,4.5,5,5.5,6,6.5},
    % legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    % y label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    label style={font=\small},
    tick label style={font=\small}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,1.64)(2,2.36)(3,2.16)
    };
% \addlegendentry{Multi Cap 1}


\addplot[
    color=black,
    mark=*,
    style=dashed,
    ]
    coordinates {
    (1,6.14)(2, 4.8)(3,3.81)
    };
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    % title={(A) Vehicle Miles Traveled},
    title={Capacity=2},
    xlabel={No of Vehicles},
    % ylabel={KMs},
    % xmin=500, xmax=2000,
    ymin=1,ymax=6.5,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={1,1.5,2,2.5,3,3.5,4,4.5,5,5.5,6,6.5},
    % legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    % y label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    label style={font=\small},
    tick label style={font=\small}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,1.27)(2,1.55)(3,1.49)
    };


\addplot[
    color=black,
    mark=*,
    style=dashed,
    ]
    coordinates {
    (1,1.91)(2, 2.31)(3,2.41)
    };

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    % title={(A) Vehicle Miles Traveled},
    title={Capacity=4},
    xlabel={No of Vehicles},
    % ylabel={KMs},
    % xmin=500, xmax=2000,
    ymin=1,ymax=6.5,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={1,1.5,2,2.5,3,3.5,4,4.5,5,5.5,6,6.5},
    % legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    % y label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    label style={font=\small},
    tick label style={font=\small}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,1.11)(2,1.22)(3,1.17)
    };

\addplot[
    color=black,
    mark=*,
    style=dashed,
    ]
    coordinates {
    (1,1.54)(2,1.76)(3,1.73)
    };

\legend{Integrated, Ride-Sharing Only}
\end{axis}
\end{tikzpicture}

\rotatebox{90}{\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,(B) Execution time}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    % title={(B) Execution time},
    xlabel={No of Vehicles},
    ylabel={Time (seconds)},
    % xmin=500, xmax=2000,
    ymin=0, ymax=50,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={0,10,20,30,40,50},
    % legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    label style={font=\small},
    tick label style={font=\small}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,10.1)(2,20.32)(3,37.23)
    };

\addplot[
    color=black,
    mark=*,
    style=dashed,
    ]
    coordinates {
    (1,3.69)(2, 7.7)(3,15.34)
    };

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    % title={(B) Execution time},
    xlabel={No of Vehicles},
    % ylabel={Time (seconds)},
    % xmin=500, xmax=2000,
    ymin=0, ymax=50,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={0,10,20,30,40,50},
    % legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    label style={font=\small},
    tick label style={font=\small}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,13.8)(2,22.81)(3,40.95)
    };

\addplot[
    color=black,
    mark=*,
    style=dashed,
    ]
    coordinates {
    (1,5.61)(2, 10.05)(3,16.37)
    };

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    % title={(B) Execution time},
    xlabel={No of Vehicles},
    % ylabel={Time (seconds)},
    % xmin=500, xmax=2000,
    ymin=0, ymax=50,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={0,10,20,30,40,50},
    % legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    label style={font=\small},
    tick label style={font=\small}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,13.73)(2,26.21)(3,39.93)
    };

\addplot[
    color=black,
    mark=*,
    style=dashed,
    ]
    coordinates {
    (1,6.55)(2,10.95)(3,18.41)
    };

\end{axis}
\end{tikzpicture}

\rotatebox{90}{\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,(C) Service Rate}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    % title={(C) Service Rate},
    xlabel={No of Vehicles},
    ylabel={Rate (\%)},
    % xmin=500, xmax=2000,
    ymin=20, ymax=100,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={0,20,40,60,80,100},
    legend pos=outer north east,
    legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    label style={font=\small},
    tick label style={font=\small},
    custom legend,
    legend style={at={(1,1.3)},anchor=south east,
        column sep=0.5em}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,72.34)(2,88.82)(3,99.97)
    };

\addplot[
    color=black,
    mark=*,
    style=dashed,
    ]
    coordinates {
    (1,23.23)(2, 51.56)(3,92.86)
    };
% \legend{Multi-Model, Mod-Only}
\end{axis}


\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    % title={(C) Service Rate},
    xlabel={No of Vehicles},
    % ylabel={Rate (\%)},
    % xmin=500, xmax=2000,
    ymin=20, ymax=100,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={0,20,40,60,80,100},
    legend pos=outer north east,
    legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    label style={font=\small},
    tick label style={font=\small}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,80.21)(2,99.85)(3,100)
    };

\addplot[
    color=black,
    mark=*,
    style=dashed,
    ]
    coordinates {
    (1,62.94)(2, 91.87)(3,100)
    };
% \legend{Multi-Modal Capacity 1,Multi-Modal Capacity 2,Multi-Modal Capacity 4,MoD-Only Capacity 1,MoD-Only Capacity 2,MoD-Only Capacity 4}
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
    width=6cm,
    % title={(C) Service Rate},
    xlabel={No of Vehicles},
    % ylabel={Rate (\%)},
    % xmin=500, xmax=2000,
    ymin=20, ymax=100,
    % xtick={500,1000,2000},
    xtick={1,2,3},
    xticklabels={{500}, {1000}, {2000}},
    ytick={0,20,40,60,80,100},
    % legend pos= south east,
    legend style={nodes={scale=0.8, transform shape}},
    ymajorgrids=true,
    grid style=dashed,
    ylabel near ticks,
    xlabel near ticks,
    label style={font=\small},
    tick label style={font=\small}
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,82.48)(2,100)(3,100)
    };

\addplot[
    color=black,
    mark=*,
    style=dashed,
    ]
    coordinates {
    (1,73.88)(2,99.03)(3,100)
    };
% \legend{Multi-Modal Capacity 1,Multi-Modal Capacity 2,Multi-Modal Capacity 4,MoD-Only Capacity 1,MoD-Only Capacity 2,MoD-Only Capacity 4}
% \legend{Multi-Model, Mod-Only}
\end{axis}


\end{tikzpicture}

\caption{Comparison of several performance metrics for varying vehicle capacities (1,2 and 4) and fleet sizes (500,1000,2000). We analyze the Vehicle Miles Traveled per served request in raw (A), execution time per iteration in raw (B), and the service rate in raw (C). The columns represent capacities 1,2 and 4 respectively.}
\label{fig:metrics}
\end{figure*}

